Mumax3-cQED: an extension of Mumax3 to simulate magnon-photon interactions in cavity QED

We present an extension of the well-known micromagnetic package Mumax3 to simulate magnon-polaritons in realistic magnetic materials and nanostructures. Mumax3-cQED leverages the full GPU-accelerated capabilities of Mumax3 to model standard spin-spin interactions and the coupling of magnetic moments to external space- and time-dependent magnetic fields, with the additional unique feature of including the coupling to a cavity. We validate the code against results obtained from the Dicke model in both the paramagnetic and the superradiant phases. We show that hybrid magnon-light states can be calculated, as well as the non-equilibrium dynamics and their approach to equilibrium. In addition, we demonstrate the potential of Mumax3-cQED to reproduce experimental results and design magnon-cavity experiments, including three-dimensional and coplanar waveguide resonators. The code is fully available and will be useful for designing experiments involving microscopic saturated ferromagnets as well as systems featuring spin textures such as domain walls, vortices, or skyrmions.

==> Makefile <==
.PHONY: all clean distclean
.SILENT: help all all-cover search-tex search-pdf

DOC := Manuscript
PUBS := publications

ifneq ($(OS),Windows_NT)
EXISTSBIBS := $(shell grep -rnw --include \*.tex '.' -e '\\bibliography{' --color=always --exclude-dir={bibliography-work-report,papers} > /dev/null && echo "true")
OUTBIBS := $(shell grep -rnw --include \*.tex '.' -e '%\\bibliography{' --color=always --exclude-dir={bibliography-work-report,papers} > /dev/null && echo "false")
SHELLBIBS := $(shell if [ "$(OUTBIBS)" = "false" ]; then echo "false"; else echo "true"; fi)
CHECKBIBS := $(shell if [ "$(EXISTSBIBS)" = "true" ]; then echo "$(SHELLBIBS)"; else echo "false"; fi)

CHECKPUBS := $(shell test -f $(PUBS).aux && echo "true")
CHECKREPORT := $(shell test -f $(DOC).pdf && echo "true")

EXISTSGLOSSARIES := $(shell grep -rnw --include \*.tex '.' -e 'makeglossaries' --color=always --exclude-dir={bibliography-work-report,papers} > /dev/null && echo "true")
OUTGLOSSARIES := $(shell grep -rnw --include \*.tex '.' -e '%\\makeglossaries' --color=always --exclude-dir={bibliography-work-report,papers} > /dev/null && echo "false")
CHECKGLOSSARIES := $(shell if [ "$(OUTGLOSSARIES)" = "false" ]; then echo "false"; else echo "true"; fi)
SHELLGLOSSARIES := $(shell if [ "$(EXISTSGLOSSARIES)" = "true" ]; then echo "$(CHECKGLOSSARIES)"; else echo "false"; fi)

OS_NAME := $(shell uname -s | tr A-Z a-z)
CHECK_DOCKER := $(shell which docker)
endif

# base compilation
base:
	pdflatex -enable-write18 --shell-escape $(DOC).tex

# compile without bibliography
nobib:
	pdflatex -draftmode -enable-write18 --shell-escape $(DOC).tex
ifeq ($(SHELLGLOSSARIES),false)
	echo "" && \
	sh -c 'echo "\033[33;1mGlossary not found !!!\033[0m"' && \
	echo ""
else
	makeglossaries $(DOC)
	echo "" && \
	sh -c 'echo "\033[33;1mGlossary found !!!\033[0m"' && \
	echo ""
endif
	pdflatex -draftmode -enable-write18 --shell-escape $(DOC).tex
	pdflatex -enable-write18 --shell-escape $(DOC).tex
	echo "" && \
	sh -c 'echo "\033[33;1mPDFLaTex compilation finished !!!\033[0m"' && \
	echo ""

# compile with index and bibliography
all:
ifeq ($(OS),Windows_NT)
	compile-latex.bat $(DOC).tex
else
	pdflatex -draftmode -enable-write18 --shell-escape $(DOC).tex
ifeq ($(SHELLGLOSSARIES),false)
	echo "" && \
	sh -c 'echo "\033[33;1mGlossary not found !!!\033[0m"' && \
	echo ""
else
	makeglossaries $(DOC)
	echo "" && \
	sh -c 'echo "\033[33;1mGlossary found !!!\033[0m"' && \
	echo ""
endif
ifeq ($(CHECKBIBS),true)
	bibtex $(DOC).aux
	echo "" && \
	sh -c 'echo "\033[33;1mBibliography found !!!\033[0m"' && \
	echo ""
else
	echo "" && \
	sh -c 'echo "\033[33;1mBibliography not found !!!\033[0m"' && \
	echo ""
endif
ifeq ($(CHECKPUBS),true)
	bibtex $(PUBS).aux
endif
	pdflatex -draftmode -enable-write18 --shell-escape $(DOC).tex
	pdflatex -enable-write18 --shell-escape $(DOC).tex
	echo "" && \
	sh -c 'echo "\033[33;1mPDFLaTex compilation finished !!!\033[0m"' && \
	echo ""
endif

bbl:
    pdflatex -enable-write18 --shell-escape $(DOC).tex
    bibtex $(DOC).aux
    pdflatex -enable-write18 --shell-escape $(DOC).tex
    pdflatex -enable-write18 --shell-escape $(DOC).tex
    make all
    
# compile with index and without bibliography
simple: nobib

# clean compilation

distclean:
	rm -f *.aux \
        $(DOC).log \
        $(DOC).blg \
        $(DOC).bbl \
        $(DOC).out \
        $(DOC).dvi \
	*.glo *.gls *.mw *.lof *.lot *.toc *.equ *.idx *.glg *.ist *.bbl *.blg

# clean compilation
clean:
ifeq ($(OS),Windows_NT)
	del /q *.aux $(DOC).log $(DOC).blg $(DOC).bbl $(DOC).out $(DOC).dvi $(DOC).pdf *.glo *.gls *.mw *.lof *.lot *.toc *.equ *.idx *.glg *.ist *.bbl *.blg >nul 2>&1
else
	rm -f *.aux \
	$(DOC).log \
	$(DOC).blg \
	$(DOC).bbl \
	$(DOC).out \
	$(DOC).dvi \
	$(DOC).pdf \
	*.glo *.gls *.mw *.lof *.lot *.toc *.equ *.idx *.glg *.ist *.bbl *.blg
endif

compile-grayscale:
	pdflatex -draftmode -enable-write18 --shell-escape "\def\forceprint{}\input{${DOC}}" $(DOC).tex
ifeq ($(SHELLGLOSSARIES),false)
	echo "" && \
	sh -c 'echo "\033[33;1mGlossary not found !!!\033[0m"' && \
	echo ""
else
	makeglossaries $(DOC)
	echo "" && \
	sh -c 'echo "\033[33;1mGlossary found !!!\033[0m"' && \
	echo ""
endif
ifeq ($(CHECKBIBS),true)
	bibtex $(DOC).aux
	echo "" && \
	sh -c 'echo "\033[33;1mBibliography found !!!\033[0m"' && \
	echo ""
else
	echo "" && \
	sh -c 'echo "\033[33;1mBibliography not found !!!\033[0m"' && \
	echo ""
endif
ifeq ($(CHECKPUBS),true)
	bibtex $(PUBS).aux
	echo "" && \
	sh -c 'echo "\033[33;1mBibliography not found !!!\033[0m"' && \
	echo ""
endif
	pdflatex -draftmode -enable-write18 --shell-escape "\def\forceprint{}\input{${DOC}}" $(DOC).tex
	pdflatex -enable-write18 --shell-escape "\def\forceprint{}\input{${DOC}}" $(DOC).tex
	echo "" && \
	sh -c 'echo "\033[33;1mPDFLaTex compilation finished !!!\033[0m"' && \
	echo ""

# compile black text but colourful images
compile-black:
	pdflatex -draftmode -enable-write18 --shell-escape "\def\compileblack{}\input{${DOC}}" $(DOC).tex
ifeq ($(SHELLGLOSSARIES),false)
	echo "" && \
	sh -c 'echo "\033[33;1mGlossary not found !!!\033[0m"' && \
	echo ""
else
	makeglossaries $(DOC)
	echo "" && \
	sh -c 'echo "\033[33;1mGlossary found !!!\033[0m"' && \
	echo ""
endif
ifeq ($(CHECKBIBS),true)
	bibtex $(DOC).aux
	echo "" && \
	sh -c 'echo "\033[33;1mBibliography found !!!\033[0m"' && \
	echo ""
else
	echo "" && \
	sh -c 'echo "\033[33;1mBibliography not found !!!\033[0m"' && \
	echo ""
endif
ifeq ($(CHECKPUBS),true)
	bibtex $(PUBS).aux
	echo "" && \
	sh -c 'echo "\033[33;1mBibliography not found !!!\033[0m"' && \
	echo ""
endif
	pdflatex -draftmode -enable-write18 --shell-escape "\def\compileblack{}\input{${DOC}}" $(DOC).tex
	pdflatex -enable-write18 --shell-escape "\def\compileblack{}\input{${DOC}}" $(DOC).tex
	echo "" && \
	sh -c 'echo "\033[33;1mPDFLaTex compilation finished !!!\033[0m"' && \
	echo ""

# convert images to black and white
print-images:
	chmod +x utils/convert-grayscale.sh && ./utils/convert-grayscale.sh && echo ""

# compile pdf and convert images to black and white
print-force: print-images compile-grayscale

# check convert imagems to grayscale
convert-grayscale: $(eval SHELL:=/bin/bash)
	@read -p $$'\e[33;1mDo you want to convert images to grayscale? [y/n]\e[0m ' -n 1 -r; \
	echo ""; \
	if [[ $$REPLY =~ ^[Yy] ]]; \
	then \
		echo "" && make print-images; \
	fi

# force print style
print: convert-grayscale compile-grayscale

# compress final pdf
compress:
	docker run --rm -v `pwd`:/pdf sergiomtzlosa/gsexiftool gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.5 -dNOPAUSE -dQUIET -dBATCH -dEmbedAllFonts=true -dPrinted=false -dSubsetFonts=true -dDetectDuplicateImages -dPDFSETTINGS=/prepress -sOutputFile=${DOC}-compress.pdf ${DOC}.pdf && \
	docker run --rm -v `pwd`:/pdf sergiomtzlosa/gsexiftool exiftool -overwrite_original -all= -tagsFromFile ${DOC}.pdf ${DOC}-compress.pdf

# extra compress
compress-big:
	docker run --rm -v `pwd`:/pdf sergiomtzlosa/gsexiftool gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/default -dPrinted=false -dNOPAUSE -dQUIET -dBATCH -dDetectDuplicateImages -dCompressFonts=true -r150 -sOutputFile=${DOC}-compress-big.pdf ${DOC}.pdf
	docker run --rm -v `pwd`:/pdf sergiomtzlosa/gsexiftool exiftool -overwrite_original -all= -tagsFromFile ${DOC}.pdf ${DOC}-compress-big.pdf

# install dependencies to convert pdf to html
# install ImageMagick 7: https://www.tecmint.com/install-imagemagick-on-debian-ubuntu/
install: install-deps
	pip install wordcloud

install-texlive:
	sudo apt-get install texlive-full

install-deps:
ifeq ($(OS_NAME),linux)
	sudo apt-get update && \
	sudo apt-get install docker python3-pygments cm-super pdfgrep poppler-utils texlive-pstricks && \
	sudo apt -y install texlive-science
endif
ifeq ($(OS_NAME),darwin)
	brew install docker pygments pdf2htmlEX pdfgrep poppler
endif

# convert pdf to html
pdf-html:
	mkdir -p html
ifeq ($(OS_NAME),linux)
	docker run -ti --rm -v `pwd`:/pdf sergiomtzlosa/pdf2htmlex pdf2htmlEX --zoom 1.5 $(DOC).pdf html/$(DOC).html
endif
ifeq ($(OS_NAME),darwin)
	pdf2htmlEX --zoom 1.5 $(DOC).pdf html/$(DOC).html
endif
	zip html/$(DOC).zip html/$(DOC).html
	rm html/$(DOC).html

# create word cloud
word-cloud:
ifeq ($(CHECKREPORT),true)
	echo "" && \
	sh -c 'echo "\033[33;1mCreating word cloud, please wait ... \033[0m"' && \
	echo "" && \
	pdftotext $(DOC).pdf - | wordcloud_cli --height 3000 --width 2000 --background white --imagefile images/wordcloud.png
endif

# compile, convert images to black and white and convert pdf to html
full-print: all print pdf-html

# compile book cover with pdflatex
cover-pdflatex:
	cd book-cover/universal && \
	pdflatex -enable-write18 --shell-escape book_cover.tex && \
	cp book_cover.pdf ../../ && \
	echo "" && \
        sh -c 'echo "\033[33;1mPDFLATEX COVER COMPILATION DONE !!!\033[0m"' && \
        echo ""

#compile cover with latex
cover-latex:
	cd book-cover/universal && \
	latex --shell-escape "\def\latexcompiler{}\input{book_cover}" book-cover/universal/book_cover.tex && \
	dvipdf -dNOSAFER -dALLOWPSTRANSPARENCY book_cover.dvi book_cover.pdf && \
	cp book_cover.pdf ../../ && \
        echo "" && \
        sh -c 'echo "\033[33;1mLATEX COVER COMPILATION DONE !!!\033[0m"' && \
        echo ""

# merge main PDF file and cover
merge-cover:
ifneq ($(CHECK_DOCKER),'')
	docker run --rm -v `pwd`:/pdf sergiomtzlosa/gsexiftool gs -dPrinted=false -sDEVICE=pdfwrite -dCompatibilityLevel=1.5 -dNOPAUSE -dQUIET -dBATCH -dEmbedAllFonts=true -dDetectDuplicateImages -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite -sOUTPUTFILE=$(DOC)-combine.pdf book_cover.pdf $(DOC).pdf && \
	echo "" && \
	sh -c 'echo "\033[33;1mPDF file + cover merged !!!\033[0m"' && \
	echo ""
else
	echo "" && \
	sh -c 'echo "\033[33;1mDOCKER NOT INSTALLED !!!\033[0m"' && \
	echo ""
endif

# reduce size main PDF
reduce-pdf:
ifneq ($(CHECK_DOCKER),'')
	docker run --rm -v `pwd`:/pdf sergiomtzlosa/gsexiftool gs -dPrinted=false -sDEVICE=pdfwrite -dCompatibilityLevel=1.5 -dNOPAUSE -dQUIET -dBATCH -dEmbedAllFonts=true -dDetectDuplicateImages -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite -sOUTPUTFILE=$(DOC)-reduced.pdf $(DOC).pdf && \
	echo "" && \
	sh -c 'echo "\033[33;1mPDF file reduced !!!\033[0m"' && \
	echo ""
else
	echo "" && \
	sh -c 'echo "\033[33;1mDOCKER NOT INSTALLED !!!\033[0m"' && \
	echo ""
endif

# compile cover and merge with main document
mm-cover: cover-latex merge-cover

# compile all with cover
all-cover: all cover-latex reduce-pdf merge-cover

# compile all with cover and word cloud
all-cover-wc: word-cloud all cover-latex merge-cover

# reduce and merge pdf file
reduce-merge-pdf: cover-latex reduce-pdf merge-cover

# search in pdf file
# USAGE: make search-pdf SEARCH_TERM=Kittel
search-pdf:
	pdfgrep -n -R "$(SEARCH_TERM)" $(DOC).pdf --exclude=bibliography-work-report | cat

# search in tex files
# USAGE: make search-tex SEARCH_TERM=Kittel
search-tex:
	grep -rnw --include \*.tex '.' -e '$(SEARCH_TERM)' --color=always --exclude-dir=bibliography-work-report | cat

# Help command
help:
	echo "" && \
	echo "Compilation help" && \
	echo "---------------------" && \
	sh -c 'echo "\033[33;1mmake base\033[0m --> Base compilation (unused)"' && \
	sh -c 'echo "\033[33;1mmake nobib\033[0m --> Full compilation without bibliography"' && \
	sh -c 'echo "\033[33;1mmake all\033[0m --> Full compilation with all latex options"' && \
	sh -c 'echo "\033[33;1mmake simple\033[0m --> Same as make nobib"' && \
	sh -c 'echo "\033[33;1mmake distclean\033[0m --> Clean compilation files"' && \
	sh -c 'echo "\033[33;1mmake clean\033[0m --> Clean compilation files and pdf file"' && \
	sh -c 'echo "\033[33;1mmake print\033[0m --> Full compilation in grayscale for printing"' && \
	sh -c 'echo "\033[33;1mmake print\033[0m --> Force full compilation in grayscale for printing"' && \
	sh -c 'echo "\033[33;1mmake compress\033[0m --> Compress output pdf"' && \
	sh -c 'echo "\033[33;1mmake compress-big\033[0m --> Strong compressing output pdf"' && \
	sh -c 'echo "\033[33;1mmake install\033[0m --> Install dependencies"' && \
	sh -c 'echo "\033[33;1mmake install-texlive\033[0m --> Install TeXLive"' && \
	sh -c 'echo "\033[33;1mmake pdf-html\033[0m --> Convert output pdf file into beautiful HTML"' && \
	sh -c 'echo "\033[33;1mmake word-cloud\033[0m --> Create a fancy word cloud image"' && \
	sh -c 'echo "\033[33;1mmake full-print\033[0m --> Compile in grayscale for printing and convert output pdf into HTML"' && \
	sh -c 'echo "\033[33;1mmake cover-pdflatex\033[0m --> Compile book cover with pdflatex"' && \
	sh -c 'echo "\033[33;1mmake cover-latex\033[0m --> Compile book cover with latex"' && \
	sh -c 'echo "\033[33;1mmake mm-cover\033[0m --> Compile book cover and merge it with output main pdf"' && \
	sh -c 'echo "\033[33;1mmake all-cover\033[0m --> Full compilation with all options, reduce size of main pdf and merge cover"' && \
	sh -c 'echo "\033[33;1mmake all-cover-wc\033[0m --> Full compilation with all options, reduce size of main pdf, merge cover and create word cloud image"' && \
	sh -c 'echo "\033[33;1mmake search-pdf SEARCH_TERM=Kittel\033[0m --> Search string in output pdf"' && \
	sh -c 'echo "\033[33;1mmake search-tex SEARCH_TERM=Kittel\033[0m --> Search string in TeX files"' && \
	sh -c 'echo "\033[33;1mmake compile-black\033[0m -->  compile black text but colourful images"' && \
	sh -c 'echo "\033[33;1mmake reduce-merge-pdf\033[0m --> Reduce pdf file and merge cover in a new pdf file"' && \
	echo ""

